ACoRe: Automated Goal-Conflict Resolution

System goals are the statements that, in the context of software requirements specification, capture how the software should behave. Many times, the understanding of stakeholders on what the system should do, as captured in the goals, can lead to different problems, from clearly contradicting goals, to more subtle situations in which the satisfaction of some goals inhibits the satisfaction of others. These latter issues, called goal divergences, are the subject of goal conflict analysis, which consists of identifying, assessing, and resolving divergences, as part of a more general activity known as goal refinement. While there exist techniques that, when requirements are expressed formally, can automatically identify and assess goal conflicts, there is currently no automated approach to support engineers in resolving identified divergences. In this paper, we present ACoRe, the first approach that automatically proposes potential resolutions to goal conflicts, in requirements specifications formally captured using linear-time temporal logic. ACoRe systematically explores syntactic modifications of the conflicting specifications, aiming at obtaining resolutions that disable previously identified conflicts, while preserving specification consistency. ACoRe integrates modern multi-objective search algorithms (in particular, NSGA-III, WBGA, and AMOSA) to produce resolutions that maintain coherence with the original conflicting specification, by searching for specifications that are either syntactically or semantically similar to the original specification. We assess ACoRe on 25 requirements specifications taken from the literature. We show that ACoRe can successfully produce various conflict resolutions for each of the analyzed case studies, including resolutions that resemble specification repairs manually provided as part of conflict analyses.

==> search-algorithms.tex <==
\section{Multi-Objective Optimization Algorithms}
\label{sec:multi-objective-search}
Several software engineering problems have been addressed by optimization algorithms~\cite{HARMAN2001833}, where such techniques could provide solutions to the difficult problems of balancing competing constraints.
Harman and Jones~\cite{HARMAN2001833} coined the term Search-Based Software Engineering (SBSE) to describe these approaches. Among them, many software engineering problems are multi-objective~\cite{Harman:2012:SSE:2379776.2379787}, in other words, the problems contain more than one fitness function to be optimized.

In contrast to a single-objective optimization problem, where there is only one global optimum solution, in a \emph{multi-objective optimization (MOO) problem} there is a set of solutions, called the \emph{Pareto-optimal} (PO) set, which are considered to be equally important, since all of them constitute global optimum solutions. 
Typically, MOO algorithms evolve the candidates population with the aim to converge to a set of non-dominated solutions as close to the true PO front as possible and maintain as diverse a solution set as possible. 

\begin{definition}[Pareto Dominance]
\label{def:pareto-dominance}
Let $S \subset U$ be a subset of individuals \red{from the universe $U$ of the} entire search-space of our interest.
Consider $f_1, \ldots, f_n$ a set of (maximizing) fitness functions, where $f_i: S \rightarrow \mathbb{R}$. 
Given two individuals $x_1$ and $x_2$, it is said that $x_1$ dominates $x_2$ if the following two conditions hold:
\begin{enumerate}[label=(\alph*)]
    \item $\forall i: 1 \leq i \leq n: f_i(x_1) \geq f_i(x_2)$
    \item $\exists i: 1 \leq i \leq n: f_i(x_1) > f_i(x_2)$
\end{enumerate}
\end{definition}
Condition (a) means that $x_1$ is not worse than $x_2$ in all objectives; while condition (2) establishes that $x_1$ is strictly better that $x_2$ at least in one objective. 

\begin{definition}[Pareto-optimal set]
\label{def:pareto-optimal-set}
Let $S \subset U$ \red{be} as before. 
The Pareto-optimal set of $S$, denoted as $PO(S)$, is the set of all non-dominated (feasible) solutions. That is, for each Pareto-optimal element $s \in PO(S)$ there is no individual in $S$ that dominates $s$.
\end{definition}


There are many variants of MOO algorithms that have been successfully applied in practice~\cite{Harman:2012:SSE:2379776.2379787}.
%Among the differences that can make one approach performs better than others, 
\red{Overall}, Figure~\ref{fig:multi-objective-search} gives an overview of how the search process is performed.
The MOO algorithm starts by creating the \emph{initial population} (step 1), composed by one or more examples of candidate individuals to be used to start the search. 
Then it iteratively performs the following steps. 
It computes the fitness value for each objective into consideration for every new individual (step 2). 
It  update the solutions set and selects the individuals that survive to the next iteration, by discarding non-promising individuals from the population set (step 3). 
To evolve and diversify the population, the algorithm creates new individuals through the application of evolution operators (step 4). The mutation operator changes (mutates) a portion of the selected individual; while the crossover operator creates new individuals by combining parts of other two individuals taken from the population (crossover is typically present in genetic algorithms). 
This evolution process is performed until some termination criterion is met, e.g., a defined number of \emph{generations} (iterations) or a maximum number of individuals are created.

\begin{figure}[htp!]
\centering
\includegraphics[width=\columnwidth]{trunk/figures/search-overview.pdf}
\vspace{-1.4em}
\caption{Multi-objective Optimization Algorithms.}
\label{fig:multi-objective-search}
\end{figure}

{\OurTool} uses a search process to look for repairs that resolve all identified goal-conflicts, \red{where the repairs} are similar to the original specification. 
\red{Overall}, {\OurTool} supports four search algorithms, namely, a \emph{Weight-based genetic algorithm (WBGA)}~\cite{DBLP:books/mit/H1992}, an \emph{Archived Multi-objective Simulated Annealing (AMOSA)} ~\cite{DBLP:journals/tec/BandyopadhyaySMD08} approach, and the \textit{Non-Dominated Sorting Genetic Algorithm III (NSGA-III)~\cite{DebJain2014}}.
We also consider an \emph{unguided search} approach that we use as a baseline during our evaluation. 
Later on Section~\ref{sec:approach} we provide further details of how {\OurTool} instantiates these MOO algorithms.

% Genetic algorithms \cite{Goldberg1989,Koza1992,Michalewicz1996} are heuristic search algorithms, inspired in natural evolution. 
% Candidate solutions are called \emph{individuals} or \emph{chromosomes}, and are often represented as sequences of \emph{genes} (characteristics) that capture their features. Genetic algorithms maintain a \emph{population} of candidate solutions, rather than a single ``current'' candidate, as in traditional search. 
% They are to a great extent driven by random decisions, e.g., in the generation of the initial population, and how the new candidate solutions are generated from existing ones. 
% To produce new individuals, it exploits information in the current population, combining their characteristics (called \emph{crossover}), or randomly altering the information in specific individuals (called \emph{mutation}). The effectiveness of this general search process is guided by a heuristic function, called \emph{fitness function}. Intuitively, this function measures how ``fit'' a particular individual is, i.e., how close it is to being an actual solution to the search problem under consideration. This evolution process is usually performed until some termination criterion is met, e.g., a defined number of iterations (known as \emph{generations} of the population).






% \subsection{NSGA-III}
% Multi-objective optimization is an area of multiple criteria decision making that is concerned with mathematical optimization problems involving two or three objective functions to be optimized simultaneously~\cite{Coello:2007evolutionary}. In general, there is more than one solution for this kind of problems. Thus, several good solutions represent the trade-off between the defined objectives.  Many-objective optimization refers to a class of optimization problems that have more than three objectives.  Multi-objective evolutionary algorithms (MOEAs), such as the Non-Dominated Sorting Genetic Algorithm II (NSGA-II)~\cite{Deb2002} and the Strength Pareto Evolutionary Algorithm 2 (SPEA2)~\cite{SPEA2}, have received immense recognition due to their effectiveness and efficiency in tackling multi-objective optimization problems. Recently, numerous studies on MOEAs revealed that when handling many-objective optimization problems, MOEAs encounter challenges and the behavior of MOEAs resembles a random walk in search space as the proportion of non-dominated solutions increases subsequently~\cite{Palakonda2020}. The Non-Dominated Sorting Genetic Algorithm III (NSGA-III)~\cite{Deb2014} was designed to solve many-objective problems and has been successfully applied. In the SBSE field, NSGA-III was also applied to solve Software Engineering many-objective problems, such as software product line testing~\cite{Jamil2019}, software remodularization~\cite{Mkaouer2015} and software refactoring~\cite{Mkaouer2014}. 



% \subsection{Genetic Algorithms}
% In most of the earlier attempts, a single objective function is constructed by combining the different objectives into one using a weighted sum approach


% Genetic algorithms \cite{Goldberg1989,Koza1992,Michalewicz1996} are heuristic search algorithms, inspired in natural evolution. 
% Candidate solutions are called \emph{individuals} or \emph{chromosomes}, and are often represented as sequences of \emph{genes} (characteristics) that capture their features. Genetic algorithms maintain a \emph{population} of candidate solutions, rather than a single ``current'' candidate, as in traditional search. 
% They are to a great extent driven by random decisions, e.g., in the generation of the initial population, and how the new candidate solutions are generated from existing ones. 
% To produce new individuals, it exploits information in the current population, combining their characteristics (called \emph{crossover}), or randomly altering the information in specific individuals (called \emph{mutation}). The effectiveness of this general search process is guided by a heuristic function, called \emph{fitness function}. Intuitively, this function measures how ``fit'' a particular individual is, i.e., how close it is to being an actual solution to the search problem under consideration. This evolution process is usually performed until some termination criterion is met, e.g., a defined number of iterations (known as \emph{generations} of the population).








% The genetic algorithms instantiate this search because they usually answer sufficiently well a broad class of problems in SBSE~\cite{Harman:2012:SSE:2379776.2379787}. In our approach, individuals represent repairs candidates, the genetic operators produce new candidates from others, and the fitness function attempts to evaluate how ``close'' a candidate is to be an optimal or sub-optimal repair. In the search, we also consider several objectives and enable settings possibilities.

\subsection{LTL Mutation and Combination}
\label{sec:ltl-mutation-crossover}
%Several operators that modify LTL formulas have been defined and used in the past. 
\red{Genetic algorithms introduced by previous studies\cite{DBLP:journals/corr/abs-2105-12595,Degiovanni+2018b}} define genetic operators, namely, mutation and crossover, to mutate LTL specifications and evolve the search. 
{\OurTool} \red{uses} this mutation operator to produce variants of goal specifications with the aim of resolving goal-conflicts. 

\begin{definition}[LTL Mutation]
\label{def:ltl-mutation}
Given an LTL formula $\phi$, function $mutate(\phi) = \phi'$ mutates $\phi$ by performing a syntactic modification driven by its syntax. 
Thus, $mutate(\phi) = \phi'$ is inductively defined as follows: 

{\fontsizeformula
\noindent
\textbf{Base Cases:}
\begin{enumerate}
\item if $\phi = \True$, then $\phi' = \False$; otherwise, $\phi' = \True$.
\item if $\phi = p$, then $\phi' = q$, where $p, q \in AP$ and $p \neq q$.
\end{enumerate}
\noindent
\textbf{Inductive Cases:}
\begin{enumerate}  \setcounter{enumi}{2}
\item if $\phi = o_{1}\phi_1$, where $o_{1} \in \lbrace \neg, \X, \F, \G \rbrace$, then:
\begin{enumerate}
	\item $\phi' = o_{1}' \phi_1$, s.t. $o_{1}' \in \lbrace \neg, \X, \F, \G \rbrace$ and $o_1 \neq o_1'$.
	\item $\phi' = \phi_1$.
	\item $\phi' = o_{1} mutate(\phi_1)$.
	\item $\phi' = q\ o_{2}'\ \phi$, where $q \in AP$ and $o_{2}' \in \lbrace \U, \W, \land, \lor \rbrace$ 
\end{enumerate}
\item if $\phi = \phi_1 o_{2} \phi_2$, where $o_{2} \in \lbrace \vee, \wedge, \U, \R, \W\rbrace$, then:
\begin{enumerate}
    \item $\phi' = \phi_1\ o_{2}'\ \phi_2$, where $o_{2}' \in \lbrace \vee, \wedge, \U, \R, \W\rbrace$ and $o_2 \neq o_2'$.
    \item $\phi' = \phi_{i}$, s.t. $\psi_{i} \in \lbrace \phi_1, \phi_2 \rbrace$ 
    \item $\phi' = mutate(\phi_1)\ o_{2}\ \phi_2$.
    \item $\phi' = \phi_1\ o_{2}\ mutate(\phi_2)$.
\end{enumerate}
\end{enumerate}
\noindent
\textbf{General Cases:}
\begin{enumerate}\setcounter{enumi}{4}
\item $\phi' = o_{1} \phi$ where $o_{1} \in \lbrace \G, \F, \X, \neg \rbrace$.
\item $\phi' = x$, where $x \in \{\True,\False\}\cup AP$
\end{enumerate}
}
\end{definition}

Base cases 1 and 2 replace constants and propositions by other constant or proposition, respectively. 
Inductive case 3 mutates unary expressions: it can change the unary operator by other (3.a), remove the operator (3.b), mutate the sub-expression (3.b), or augment the current formula by including a binary operator and a proposition (3.d). 
Inductive case 4 mutates binary expressions: it can change the binary operator (4.a), remove one of the expressions and the operator (4.b), or mutate one of the sub-expressions (4.c and 4.d).
Cases 5 and 6 are more general in which the entire formula $\phi$ is augmented with one unary operator (5) or replaced by a constant or proposition (6).

\begin{figure}[htp!]
\centering
\includegraphics[width=.6\columnwidth]{trunk/figures/mutants.pdf}
\caption{Examples of the mutations that {\OurTool} implements.}
\label{fig:mutants}
\end{figure}

Figure~\ref{fig:mutants} shows 5 possible mutations that can be generated for formula $\F (p \Implies \G r)$. 
Mutant M1 replaces $\F$ by $\G$, leading to $M1:\G (p \Implies \G r)$.
Mutant $M2:\F (p \land \G r)$ replaces $\Implies$ by $\land$. 
Mutant $M3:\F (p \Implies \neg r)$ replaces $\G$ by $\neg$.
Mutant $M4: \F (true \Implies \G r)$, reduces to $\F \G r$,  replaces $p$ by $\True$. 
While mutant $M5 : \F (p \Implies \G q)$ replaces $r$ by $q$.


Typically, genetic algorithms that manipulate LTL formulas also implement a crossover operator~\cite{DBLP:journals/corr/abs-2105-12595,Degiovanni+2018b}. 
This operator takes two LTL formulas $\phi$ and $\psi$, and produces a new formula combining parts of both $\phi$ and $\psi$. 
This operator will later be used by the two variants of genetic algorithms that {\OurTool} integrates, namely a\emph{Weight-based genetic algorithm (WBGA)}~\cite{DBLP:books/mit/H1992} and  the Non-Dominated Sorting Genetic Algorithm III (NSGA-III)~\cite{DebJain2014}.

\begin{definition}[LTL Combination]
\label{def:ltl-crossover}
Let $\phi$ and $\psi$ two LTL formulas. Function $combine(\phi,\psi) $ will produce the new formula $\phi'$ by performing the following steps:
\begin{enumerate}
    \item It selects a sub-formula $\alpha$ from formula $\phi$; to be combined;
    \item it selects sub-formula $\beta$ from $\psi$;
    \item it either, (a) $\phi'= \phi[\alpha \mapsto \beta]$ replaces $\alpha$ by $\beta$ in $\phi$; or (b) $\phi'= \phi[\alpha \mapsto \alpha\ o_2\ \beta]$ combines $\alpha$ and $\beta$ with a binary operator $o_{2} \in \lbrace \vee, \wedge, \U, \R, \W\rbrace$.
\end{enumerate}
\end{definition}

\begin{figure}[htp!]
\centering
\includegraphics[width=\columnwidth]{trunk/figures/combination.pdf}
\vspace{-1.4em}
\caption{Examples of the combinations that {\OurTool} implements.}
\label{fig:crossover}
\end{figure}

\red{Figure~\ref{fig:crossover} provides an illustration of how} this operator works in case a (i.e., option 3.a).
In this example $\phi:\F (p \Implies \G r)$ and $\psi:\neg p \land q$. The selected formulas are $\alpha: p$ and $\beta:\neg p$. 
Thus, $combine(\phi,\psi)$ returns $\phi': \F (\neg p \Implies \G r)$.


==> threat-to-validity.tex <==
\section{Threat to Validity}
\label{sec:threat-to-validity}
Threats to external validity may be related to the case studies and specifications we used in our evaluation. 
To mitigate this threat, we searched for independent specifications taken from the literature and benchmarks, that are typically used for evaluation requirements analysis tools. Although results may not generalize to other specifications and domains (for instance, when a different specification language than LTL is employed).

Threats to internal validity concern the implementation steps. 
%For instance, we re-implemented an established exact model counter to validate our approximate model counting method, which we validated by manually checking the results for several examples. 
Regarding the implementation of our approach, which includes third-party libraries, we mitigate this risk through several repetitions of various experiments and the adoption of reliable libraries. 
Particularly, the multi-objective algorithms contain an elevated degree of randomness in their search process. For instance, the application of the evolutionary operators is completely dependent of random decisions. 
To mitigate this threat, we repeat our experiments 10 times, following traditional research guidelines of how random algorithms should be evaluated~\cite{RandomizedArcuri}, to reduce potential threats raised by the random elections of the search algorithms.

Our assessment metrics, the number of repairs in the Pareto-optimal set and not introducing new conflicts, are intuitive and reflect the effectiveness of {\OurTool}. 
Moreover, the quality indicators (such as the hypervolume (HV) and inverted generational distance (IGD)) are a standard way to compare multi-objective search algorithms. 
We also employ several non-parametric statistical tests (namely, Kruskal–Wallis H-test and Vargha and Delaney's $\hat{A}_{12}$) to assess \blue{if the algorithm performs significantly different from each other.}

Although the mentioned threats, 
\iffalse 
we are confident that the results will remain in other case studies.
\fi
{\OurTool} can successfully produce several repairs, that require the validation by part of a domain expert. 
In this work, we did not focus on the ``readability'' of the repairs or the comprehension from the point of view of engineers, but we use the syntactic similarity metric as a proxy for these properties. \blue{Regarding future work, we intend to conduct qualitative studies that involve experienced developers. %in future works.
Additionally, all} the mentioned limitations present an interesting direction that we hope to follow in future work.
